Linear Policies are Sufficient to Realize Robust Bipedal Walking on Challenging Terrains

In this work, we demonstrate robust walking in the bipedal robot Digit on uneven terrains by just learning a single linear policy. In particular, we propose a new control pipeline, wherein the high-level trajectory modulator shapes the end-foot ellipsoidal trajectories, and the low-level gait controller regulates the torso and ankle orientation. The foot-trajectory modulator uses a linear policy and the regulator uses a linear PD control law. As opposed to neural network-based policies, the proposed linear policy has only 13 learnable parameters, thereby not only guaranteeing sample efficient learning but also enabling simplicity and interpretability of the policy. This is achieved with no loss of performance on challenging terrains like slopes, stairs and outdoor landscapes. We first demonstrate robust walking in the custom simulation environment, MuJoCo, and then directly transfer to hardware with no modification of the control pipeline. We subject the biped to a series of pushes and terrain height changes, both indoors and outdoors, thereby validating the presented work.

==> Sections/Introduction_v1.tex <==
% issue 1: quadruped controllers dont extend well to bipeds. why? they use a simplified model. make assumptions: single potato model

% issue 2: exising controllers fo rbipeds are complex and layered, HZD + raibert's controller, DNN + (Michel Van de penne 's work), several concepts are combined to get a walking controller. 

% In our approach we would follow a methodology where there are no simplications of the model, and yet use a light-weight control framework that can be learned via RL.  So we use end-foot trajectoroes modulated, .... 

% not making assumptions
% simple policy
% unified framework

% combining these two
% full scale biped
% transferability
% semi ellipses

\section{Introduction}

 Locomotion for legged robots has been an active field of research for the past decade owing to the rapid progress in actuator and sensing modules. Actuators like the BLDC motors have become efficient and powerful, and sensors like the IMUs have become more accurate and affordable. As a result, there has been a spurt in the growth of high performance legged robots over the last few years \cite{Bledt2018MIT,Leeeabc5986}. In particular, there has been rapid progress in the domain of quadrupedal robots, and there is a general push for the realization of natural and efficient locomotion behaviours comparable with animals. For example, the MIT Cheetah uses a combination of Model Predictive Control (MPC) and whole-body impulse control, enabling it to walk on rough terrains and generate back-flips \cite{Bledt2018MIT}. Similar controllers are in use for Spot from Boston Dynamics, Vision 60 from Ghost Robotics and others. However, these controllers, despite being successful, are using a simplified model (the ``single potato" model), which is not applicable for bipeds. Hence, the controller development for bipeds and quadrupeds have largely had their own separate paths. 
% have not yet been deployed in bipeds successfully. The bipeds generally fail to satisfy the single body assumption and have significant deviations from the domain of quadrupedal systems.

% Even with such progress, the controllers don't extend well to bipeds. Quadrupedal locomotion strategies have been based on simplified models with unified single rigid body assumptions like the ``space potato model'' of MIT Cheetah \cite{Bledt2018MIT}. The appearance of sophisticated bipedal robots fail to satisfy the unified body assumption and hence have significant deviations from quadrupedal systems.

\begin{figure}[!t]
\centering
\vspace{2mm}

\includegraphics[width =0.9\linewidth]{Figures/BipedImages/intro_train_3.png}
\caption{Figure showing Rabbit (Top) and Digit (Bottom) in Simulation: Traversing incline and decline with robustness towards adversarial forces}
\label{fig:intro_train}
\vspace{-5mm}
\end{figure}

While numerous works have demonstrated successful bipedal controllers, effective bipedal locomotion strategies which accomplish robust walking on rough terrains are heavily engineered and layered, consisting of several concepts being stacked to get a stable walking controller. For example, SLIP models in conjunction with Raibert's controller are used to achieve stable walking \cite{apgar2018rss}.
%Other models include using centroidal models based on Raibert's controller \cite{raibert1986legged},
Other methods include the centroidal models, the Zero-Moment Point (ZMP) \cite{tedrake2004}, the linear inverted pendulum \cite{gong2020angular}, and Hybrid Zero Dynamics (HZD) \cite{hzd_grizzle}. They are usually combined with either offline or online trajectory optimization to obtain a library of behaviors \cite{heried2018cfrost,xiong2018ames}. While the offline optimization uses the full body model, the online part uses an approximate model in order to solve it in real-time. % or feedback linearization \cite{gongetal2018}
% are well known. 
% On the one hand, Model Predictive Control (MPC) \cite{powell2015icra}, and Hybrid Zero Dynamics (HZD), \cite{hzd_grizzle} modeling the underlying dynamics more accurately tend to yield more natural dynamic walking behaviors.
% Recently, \cite{gong2020angular} utilizes the Angular momentum-based LIP controller to achieve agile walking on irregular terrains with significant elevation (wavefield). 


Apart from the classical approaches that are heavily influenced by model based design, Reinforcement Learning (RL) based approaches have gained popularity today \cite{guillermo3D,siekmann2020learning,2020-ALLSTEPS,deeploco}. %, wherein the idea is to let the robot learn to walk by itself. 
Physics-based bipedal character animation \cite{deeploco} has shown benefits of using Deep Reinforcement Learning (DRL) algorithms by generating robust locomotion strategies for a diverse set of terrains. \cite{cdmloco} learned centroidal dynamics based motion planners for multi-legged systems in rough terrain by using DRL stacked with their inverted pendulum on cart (IPC) model. Similarly \cite{siekmann2020learning}, \cite{cassie2019sim2real} use novel DRL frameworks for walking on flat terrain and present a direct policy transfer of learned strategies from simulation to a physical robot.
% However, unlike the robot used in \cite{gong2020angular}(Cassie), robot platforms discussed in this work have significant torso inertia and require separate terrain relative torso adaptation strategies.
% 
% Most state-of-the-art approaches employ Deep Reinforcement Learning (DRL) algorithms to enhance various aspects of bipedal locomotion. 
%Such methods ensure that the policy converges to a more practical solution using reference trajectories  \cite{deeploco} and have not yet shown to be suitable for physical robots.
% However, their hardware transferability to practical bipedal robots has not yet been demonstrated. 
%\cite{cassie2019sim2real} used a DRL framework for walking on flat terrain and presented a direct policy transfer from generating learned strategies from simulation to a physical robot.
Also, some of the works like
\cite{guillermo3D,da2019grizzle} have focused on blending the classical and learning based approaches. 
 % used supervised learning to blend all the concepts mentioned earlier to control the high-dimensional bipedal system based on a low-dimensional surface of the system's state space. 
% Such DRL-based policies are computationally intensive and were not shown to generalize to rough terrain walking. 
% Usage of reference motions \cite{siekmann2020learning} or a non-random sub-optimal initial policy could significantly leverage the sample efficiency and reduce the burden on the learning algorithm. 
However, all of the approaches mentioned are computationally intensive, requiring several thousands of parameters for the neural network policy. In this paper, we would like to develop a control framework that neither uses extensive dynamic modeling, nor uses simplifying assumptions (like in quadrupeds). More importantly, we would like to use control policies that are computationally less intensive.

% However, obtaining such reference motion could be tiresome, and the development of sub-optimal initial policies through behavioral cloning \cite{paigwar2020robust} is not straightforward and is often as difficult as the learning itself. 
% Recently, \cite{guillermo2D, guillermo3D} explored HZD based RL framework for developing robust flat ground walking using small-scale neural networks.


\subsection{Contributions and Paper Organization}

Our primary focus in this paper is walking on varying slopes and elevated terrains, which bring in a new set of challenges. We would like to follow a methodology similar to \cite{Leeeabc5986}, which uses a high-level policy that shifts the end-foot trajectories to realize robust walking on a diverse set of terrains. In particular, we propose a  formulation for bipedal locomotion that generates linear control policies, that not only transform the semi-elliptical trajectories, but also reshape them.
%modulating the properties of a  semi-elliptical end-foot trajectory.
This was used to realize robust walking in the quadrupedal robot, Stoch 2, in simulation \cite{paigwar2020robust}. Based on the support plane and torso orientation, appropriate trajectories are generated,
%these trajectories are reshaped and transformed, 
which are then tracked via a joint level PD control law. With a structured low-level tracking controller, the policy is freed from learning the joint level coordination and non-linear control relations, thus making our approach intuitive. 
%To our knowledge, our work is the first to demonstrate robust bipedal walking with a highly compute-efficient linear control policy on realistic robot platforms. 
The contributions of the paper are as follows:

\textbf{Low computational overhead:} The main contribution of this paper is on training robust bipedal walking on challenging terrains with low computational footprint. By incorporating the priors of bipedal walking strategies and formulating a relevant control structure,  we significantly decrease the number of learnable parameters to  9 for Rabbit (2D) and 80 for Digit (3D). Our linear control policies are considerably compact compared to even the smallest of the neural network policies \cite{guillermo3D} capable of 3D bipedal walking. We firmly believe that having such a simplistic linear policy will greatly leverage our policy's explainability compared to any of the previous works,  \cite{cassie2019sim2real}, \cite{siekmann2020learning}. This feature allows us to obtain intuitive seed policies that enhance the sample efficiency of learning and realization of practical walking behaviours.

\textbf{Unified framework:} We previously achieved robust locomotion via linear policies in quadrupeds \cite{paigwar2020robust}.  Given the success behind this policy, we focused on implementing this methodology in bipeds, which are much harder to control. More importantly, bipeds have feet, which play a major role in stabilizing the torso. We have a unified learning-based control framework deployed alike for quadrupeds and bipeds. 

\textbf{Robustness and generalization:} We demonstrate walking on slopes of up to $20\degree$, walking backwards, and with feet. Our controller can reject disturbances, adapt to terrain transitions, and recover from adversarial force perturbations up to $120$ N. We validate our results on two bipedal robots, Rabbit and Digit, in simulation and show preliminary transfer of the policies in Digit hardware.

The paper is structured as follows: Section \ref{sec:background} will provide the description of the robot test-beds and the associated hardware considerations. Section \ref{sec:approach} will describe the control framework for the proposed strategy, followed by the description of the training process used in Section \ref{sec:training_eval}. Finally, the simulation results will be discussed in Section \ref{sec:simulation_results}.
% and \ref{sec:conclusion}.



% The paper is structured as follows: Section \ref{sec:background} will provide the description of the robot test-beds and the associated hardware considerations. Section \ref{sec:approach} will describe the control framework for the proposed strategy, followed by the description of the training process used, in Section \ref{sec:training_eval}. Finally, the simulation results and preliminary transfer of the framework to hardware will be discussed in Section \ref{sec:simulation_results} and Section \ref{sec:conclusion} respectively.

